En Route Path-planning for Partially Occupied Vehicles in Ride-pooling Systems

Ride-pooling services, such as UberPool and Lyft Shared Saver, enable a single vehicle to serve multiple customers within one shared trip. Efficient path-planning algorithms are crucial for improving the performance of such systems. For partially occupied vehicles with available capacity, we introduce a novel routing algorithm designed to maximize the likelihood of picking up additional passengers while serving the current passengers to their destination. Unlike traditional methods that group passengers and vehicles based on predefined time windows, our algorithm allows for immediate responses to passenger requests. Our approach optimizes travel time while dynamically considering passenger demand and coordinating with other vehicles. Formulated as an integer linear programming (ILP) problem, our method is computationally efficient and suitable for real-time applications. Simulation results demonstrate that our proposed method can significantly enhance service quality.

==> ieeeconf/sec/Attractiveness.tex <==
\subsection{Attractiveness: Passenger Demand}\label{sec: attractiveness}

The road network is represented by a graph $G = (Q, E, \omega)$, where $Q$ is the set of nodes (road intersections), $E$ is the set of edges (road segments) and $\omega$ is the length of each road segment accordingly. Given the historical trip data, we can estimate the passenger arrival with Poisson parameter $\lambda^t(i,j)$, which is the destination-$j$-specific Poisson arrival of customers at node $i$ at time $t$, where $i,j \in Q$.
 % A request can be described by a tuple including the origin, the destination, and the time when the request is sent out.

 A passenger request can be modeled through a pair $(O^A, D^A)\in Q\times Q$, where $O^A$ and $D^A$ represent the origin and destination nodes, respectively, with $O^A \neq D^A$. 
Considering the current trip $\{O^A, D^A\}$, the adjusted Poisson arrival of passenger in location $i$ is defined as follows
\begin{equation}\label{attractiveness}
    \lambda_{Att}^t(i, O^A, D^A) = \sum_{j\in Q}\lambda^t(i,j)  \frac{\mathcal{L}_s(O^A, D^A)+ \mathcal{L}_s( i,j)}{2\mathcal{L}_p (O^A, D^A, i, j)},
\end{equation}
where $\mathcal{L}_s(i,j)$ is a function that returns the traveling distance if a vehicle travels directly from node $i$ to $j$ following the shortest path calculated by Floyd-Warshall Algorithm \cite{Floyd1962}. 

In this work, we consider two possible shared traveling sequences for ride-pooling: $O^A \rightarrow O^B \rightarrow D^A \rightarrow D^B$ (first pick-up, first drop-off) and $O^A \rightarrow O^B \rightarrow D^B \rightarrow D^A$ (first pick-up, last drop-off). $\mathcal{L}_p(O^A, D^A, i, j)$ returns the minimal total traveling distance when passenger $A$ shares a ride with another passenger from origin $i$ to destination $j$. It is defined as:
% \begin{equation}\label{detourdist}
% \footnotesize	
% \mathcal{L}^d(O^A, D^A, i, j) =\\
% \min \left\{
% \begin{aligned}
% & \mathcal{L}_s(O^A, i) + \mathcal{L}_s(i, j) + \mathcal{L}_s(j, D^A), \\
% & \mathcal{L}_s(O^A, i) + \mathcal{L}_s(i, D^A) + \mathcal{L}_s(D^A, j)
% \end{aligned}
% \right\}
% \end{equation}
\begin{equation}\label{detourdist}
% \footnotesize	
\begin{aligned}
\mathcal{L}_p(O^A, D^A, i, j) =
\min \{
 \mathcal{L}_s(O^A, i) + \mathcal{L}_s(i, j) + \mathcal{L}_s(j, D^A),& \\
 \mathcal{L}_s(O^A, i) + \mathcal{L}_s(i, D^A) + \mathcal{L}_s(D^A, j)\}&
\end{aligned}
\end{equation}
The numerator $ \mathcal{L}_s(O^A, D^A) + \mathcal{L}_s(i, j)$ in~\eqref{attractiveness} represents the sum of the individual shortest path distances for both passengers if they were to travel solely/separately. The ratio {\large $ \frac{\mathcal{L}_s(i, j) + \mathcal{L}_s(O^A, D^A)}{2\mathcal{L}_p(O^A, D^A, i, j)}$} $\in (0, 1]$ quantifies the efficiency of pooling the ride, that a larger detour increases $\mathcal{L}_p (O^A, D^A, i, j)$. For example, when trips from node $i$ are in the opposite direction of trip ${O^A, D^A}$, this results in a smaller ratio, making node $i$ less attractive for picking up an additional passenger.



% \begin{equation}\label{attractiveness}
%     \lambda_{Att}^t(i, O^A, D^A) = \sum_{j\in Q}\lambda^t_{OD}(i,j)  \frac{2 \cdot min\left\{\mathcal{L}_s(i, j), \mathcal{L}_s(i, D^A)\right\} }{\mathcal{L}_s(O^A, D^A)+ \mathcal{L}_s( i,j)},
% \end{equation}

% The larger the detour is, the smaller $ \frac{\mathcal{L}_s(t, i,j) + \mathcal{L}_s(t,O^A, D^A)}{\mathcal{L}^d (O^A, D^A, i, j)}$ will be, thus the less attractive the node $i$ will be for picking up an additional passenger.

% A larger detour increase ${\mathcal{L}^d (O^A, D^A, i, j)}$, e.g., trip $(i, j)$ traveling to the opposite direction of trip $O^A, D^A$, making the ratio smaller, thus the less attractive the node $i$ will be for picking up an additional passenger.



==> ieeeconf/sec/Repulsiveness.tex <==
\subsection{Repulsiveness: Other vehicles}\label{sec: Repulsiveness}
Inspired by the matching function considered in \cite{Buchholz2021} and the empirical law of pooling-matching probability found in \cite{Ke2021}, we formulate the probability of a match for a partially occupied vehicle at node $i$ as follows
% \subsubsection{Match probability}
% Inspired by \cite{Buchholz2021}, the probability of a match form a not-fully occupied AV's perspective in location $i$ is given by
\begin{equation}
    p^t_{node}(i, O^A, D^A) = 1- \zeta exp \left(- \frac{\lambda_{Att}^t(i, O^A, D^A)}{\eta n^t(i)}\right),
\end{equation}
% where $\eta$ is region-specific as it reflects the difficulty of search within a region, e.g., the complexity of the street grid. 
where $\eta$ is a region-specific positive parameter related to the difficulty of searching available vehicles, influenced by factors such as the network structure. 
% This parameter reflects the physical characteristics of a region and is usually assumed to remain fixed throughout the day. 
% They are physical characteristics of a region which are assumed to be fixed across the day. 
Since our matching scheme is operated through a centralized cloud platform, we use a uniform value of $\eta$ across all nodes. $\zeta \in (0,1]$ is a parameter related to the matching radius and passengers’ and vehicles’ distribution. $\lambda_{Att}^t$ is the adjusted Poisson arrival rate of passengers, as defined in~\eqref{attractiveness}. $n^t(i)$ is the number of available vehicles surrounding node $i$ within a matching radius $d_{match}$ at time $t$, calculated as:
\begin{equation}
    n^t(i) = n^t_{empty}(i) + n^t_{drop}(i) + 0.5 n^t_{partial}(i) ,
\end{equation}
where captures the effective number of available vehicles near node $i$, accounting for different levels of availability. Empty vehicles, represented by $n^t_{empty}(i)$, are fully available for new passenger requests. Vehicles in the process of dropping off their final passenger, $n^t_{drop}(i)$, will soon be available once they reach their destinations.
% are also weighted by a factor of 0.5, reflecting that they will soon be available but are not immediately accessible. 
Partially occupied vehicles, denoted by $n^t_{partial}(i)$, are assigned a multiplier of $0.5$, as they can only accept one additional passenger. 
% This weighted approach allows the model to more accurately represent real-time vehicle availability, crucial for effective matching in ride-pooling scenarios.


% which measures the number of empty vehicles and partially occupied ones, where a multiplier of $0.5$ is given to the later to account for their partial availability. It also considers the vehicles which are currently completing a trip and dropping off their final passenger. They are also weighted by a factor of 0.5, as they will become fully available shortly but are not immediately accessible.





% Then, the probability of a match event occurring at the road segment $edge_{i,j} \in E$, whose start and end intersections are node $i$ and $j$ respectively, is defined as the average match probability at the edge’s start and end intersections:
% \begin{equation}
%     p(i,j) = \frac{prob(i,O^A, D^A, n^t) + prob(j, O^A, D^A, n^t)}{2}
% \end{equation}
% This approach averages the match probabilities at nodes $i$ and $j$, providing a balanced estimate of the likelihood of a match occurring anywhere along the segment. The assumption of equal contribution from both nodes simplifies the computation and reflects a symmetric influence on match probability across the segment.
\subsection{Likelihood of getting a second passenger on edge}
Assuming that the start and end nodes contribute equally to a potential match on a road segment, the probability of a match event occurring on the edge $(i,j) \in E$, starting at node $i$ and ending at $j$, is defined as:
\begin{equation}
\footnotesize
p^t_{edge}(i, j, O^A, D^A) = \left(p^t_{node}(i, O^A, D^A) + p^t_{node}(j, O^A, D^A)\right)/2.
\end{equation}
% \begin{equation}
% \begin{aligned}
% p^t_{edge}(i, j, O^A, D^A) = &(p^t_{node}(i, O^A, D^A)\\
% &+ p^t_{node}(j, O^A, D^A))/2.
% \end{aligned}
% \end{equation}


For clarity, we simplify $p^t_{edge}(i, j, O^A, D^A)$ to $p^t(i,j)$ in the following sections.
The travel time on edge $(i, j)$ can be estimated using measurement methods such as infrared loop detector, historical data, or real-time vehicle GPS trajectories \cite{Wang2014}, denoted as $\hat{T}(i, j)$. By assuming that match opportunities occur independently over time, the probability of not obtaining a match during the travel time $\hat{T}(i, j)$ is $(1 - p^t(i,j))^{\hat{T}(i,j)}$. Therefore, the probability of a partially occupied vehicle picking up a second passenger while traveling along edge $(i, j)$ is given by
\begin{equation}\label{eq: edge_prob}
\mathcal{P}^t_{ij} = 1 - (1 - p^t(i,j))^{\hat{T}(i,j)}.
\end{equation}
% \vspace{+0.1cm}

% This expression accounts for the cumulative probability of finding a match over the entire duration of the trip along edge $(i, j)$, reflecting an increased likelihood of a match as the vehicle spends more time on the segment.

